Monotone Boolean Functions, Feasibility/Infeasibility, LP-type problems and MaxCon

This paper outlines connections between Monotone Boolean Functions, LP-Type problems and the Maximum Consensus Problem. The latter refers to a particular type of robust fitting characterisation, popular in Computer Vision (MaxCon). Indeed, this is our main motivation but we believe the results of the study of these connections are more widely applicable to LP-type problems (at least 'thresholded versions', as we describe), and perhaps even more widely. We illustrate, with examples from Computer Vision, how the resulting perspectives suggest new algorithms. Indeed, we focus, in the experimental part, on how the Influence (a property of Boolean Functions that takes on a special form if the function is Monotone) can guide a search for the MaxCon solution.

==> MBFfig.tex <==
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.4\textwidth]{extrafigs/4cube.pdf}  
\end{center}

\caption{\label{MBFfig} Boolean Cube and MBF}
The Boolean Cube is a generalisation of the 2D unit square (vertices (0,0), (0,1), (1,0) and (1,1)). 
The 4D Boolean Cube is drawn flattened onto 2D; and oriented so that the higher up a vertex appears, the larger is the number of 1's in the coordinates.

Interpreting the bits as coding membership in a set associated with that vertex (bit $i$ set to one if element $i$ belongs in the subset) relates the Boolean Cube to the Hasse Diagram (ordering of subsets by inclusion). In essence, the Boolean cube is this diagram ``without the arrowheads''.

A Boolean Function maps the Boolean cube to 0 or 1. We illustrate by colouring:  ``white''  nodes map to 0, coloured node (see the text below for explanation of the different colours) map to 1.

This example is a {\em Monotone} Boolean Function: moving up the picture, the value of the function only ever increases, it {\em never} transitions in the opposite direction.
\end{figure}

